Formal Language Theory Meets Modern NLP

NLP is deeply intertwined with the formal study of language, both conceptually and historically. Arguably, this connection goes all the way back to Chomsky's Syntactic Structures in 1957. It also still holds true today, with a strand of recent works building formal analysis of modern neural networks methods in terms of formal languages. In this document, I aim to explain background about formal languages as they relate to this recent work. I will by necessity ignore large parts of the rich history of this field, instead focusing on concepts connecting to modern deep learning-based NLP.

==> ntks.tex <==
\section{Neural tangent kernels}

TODO: Is it worth discussing these here? Should probably just refer to other people

Much recent work in deep learning theory has identified the \emph{neural tangent kernel} (NTK) as an interesting abstraction for understanding the generalization properties of very wide neural nets.
